Recent Developments in Security-Constrained AC Optimal Power Flow: Overview of Challenge 1 in the ARPA-E Grid Optimization Competition

The optimal power flow problem is central to many tasks in the design and operation of electric power grids. This problem seeks the minimum cost operating point for an electric power grid while satisfying both engineering requirements and physical laws describing how power flows through the electric network. By additionally considering the possibility of component failures and using an accurate AC power flow model of the electric network, the security-constrained AC optimal power flow (SC-AC-OPF) problem is of paramount practical relevance. To assess recent progress in solution algorithms for SC-AC-OPF problems and spur new innovations, the U.S. Department of Energy's Advanced Research Projects Agency--Energy (ARPA-E) organized Challenge 1 of the Grid Optimization (GO) competition. This paper describes the SC-AC-OPF problem formulation used in the competition, overviews historical developments and the state of the art in SC-AC-OPF algorithms, discusses the competition, and summarizes the algorithms used by the top three teams in Challenge 1 of the GO Competition (Teams gollnlp, GO-SNIP, and GMI-GO).

==> src/EC_difficulty.tex <==
\section{Measuring Challenge 1 Problem Difficulty}
\label{sec:difficulty_assesment}

The gap between an upper and a lower bound is a conventional way of measuring the quality of a result. Furthermore, a problem with a small gap for a given run time is presumed easier than a problem with a larger gap in the same time. The bounds for Challenge results are not known, but there is a range of results for the best solutions of a given scenario. Considering the best results, when the gap between them is small, it is likely that the solution was easier to obtain than when the gap is larger. Therefore, we define a gap $\epsilon$ as $$\epsilon = \frac{O_2}{O_1} - 1$$
where $O_1$ is the best objective value obtained and $O_2$ is the second best. The ``Wisdom of the Crowd'' technique dates from Aristotle and relies on ``noise cancellation'', where the larger the set the less likely a bad result. The set under consideration is the 350 synthetic scenario results produced by 26 teams across 4 scoring divisions. Since this is an a posteriori approach, it cannot be used to select a set of scenarios with a range of difficulties, a desirable attribute in a competition.

For selecting the scenarios for competition use, Carleton Coffrin developed a \emph{hardness} index, $H$, that is the product of 3 values calculated using the benchmark program for Division 2:
\begin{itemize}
    \item Relative cost, $C^r$, the difference of DC-SCOPF and AC-SCOPF generation cost normalized by the AC-SCOPF cost value
    \item Relative penalty, $P^r$, the AC penalty value divided by the cost
    \item $\log_{10}$ of a relative upper bound penalty, $P^{ubr}$, the AC penalty upper bound divided by the cost
\end{itemize}
$$H = C^r P^r \log_{10}(P^{ubr})$$
Unfortunately, the index breaks down completely for the larger cases (networks 20, 25, and 30), partially on some other networks (75 and 82) so some approximations were made in these cases. The final selection aimed for a distribution of Hardness values.

Direct comparison of individual gap $\epsilon$ and hardness $H$ values was not very successful, with the Pearson value dropping to a rather insignificant $0.18$, but after pruning about a third of the scenarios the Pearson coefficient came back up to $0.75$.

\begin{table}
    \centering
    \caption{Distribution of synthetic gap $\epsilon$ and hardness $H$ values. $1.95 \times 10^{-5} \leq \epsilon \leq 3.69$, Pearson coefficient 0.94.}
    \label{tab:hardness}
    \begin{tabular}{|c|c|c|}
        \hline
        Value range & Gap $\epsilon$ count & Hardness $H$ count \\ \hline
        $[0.0, 10^{-3})$ & 6 & 8 \\
        $[10^{-3}, 10^{-2})$ & 28 & 42 \\
        $[10^{-2}, 10^{-1})$ & 162 & 110 \\
        $[10^{-3}, 10^{-2})$ & 128 & 132 \\
        $[10^{-3}, 10^{-2})$ & 16 & 45 \\
        $[10^{-3}, 10^{-2})$ & 0 & 3 \\ \hline
    \end{tabular}
\end{table}

==> src/platform.tex <==
% Platform Observations, Challenges
% Arun Veeramany

% Note to Ignacio et al. - Feel Free to cut down irrelevant content


\section{Competition Platform}

\subsection{Competition Submission Workflow}
\label{S:workflow}


\begin{figure}[htbp]
\centerline{\includegraphics[scale=0.33]{go-images/GO-diagrams-work-flow.png}}
\caption{\label{fig:SysWorkflow} Competition Submission Workflow Summary}
\end{figure}

{\bf Figure \ref{fig:SysWorkflow}} shows how an entrant team's submission is managed. The process begins on the Team Submission page on the External web site where a member of a team makes a submission for an open challenge. The entrant selects a few items, including language, GitHub repository details, choice of divisions, and data set against which this submission needs to run. In Challenge 1 prizes were awarded in four divisions. Division 1 (Real-Time) had a 10-minute limit to solve the base case given a reasonable starting point and Division 2 (Off-line) had a 45-minute limit to solve the base case given no starting point information. Scoring is based on the lowest cost (objective value). Divisions 3 and 4 use the same data sets as Divisions 1 and 2 but are scored using a performance profile model \cite{Dolan2002PerformanceProfiles} instead of the lowest cost model. Performance profiles are calculated outside the evaluation platform but using the lowest cost scores generated by the platform for Divisions 3 and 4. Different algorithms could be used in the performance profile divisions and the lowest cost divisions.
More details are provided in Section~\ref{sec:platform-details}.


\subsection{Evaluation Platform}
\label{S:Cluster}

Each team was allowed to use up to six nodes for parallel computing throughout the Competition be it for their Sandbox testing or for any of the Challenge events owing to several benefits that supercomputing clusters bring to the advancement of science and engineering. Constance is the hosting organization's institutional computing cluster based on the Intel Haswell CPU architecture. Though 520 compute nodes were available, these needed to be shared with rest of the organization. Therefore, the supply of nodes was always variable depending on  organization-wide demand. Scenario and scoring schedulers were constantly running on one of the login nodes as a  background process. These were bash scripts that invoked web services to receive next scenario to be run from the pending list. 

Entrant codes 1 and 2 were launched one at a time using SLURM commands in a blocking mode. Apart from time limits imposed by the Competition, the command line options included entrant choices obtained through their respective submission.conf. There were a variety of requests for resource allocation with an upper Competition-prescribed limit of six nodes: 
    (1) single node,
    (2) all six nodes,
    (3) all 144 cores (24 cores per node times 6 nodes),
    (4) six nodes and less than 24 cores per node, and
    (5) different set of requirements for code1 and code2


Entrants were allowed to export system, MPI implementation and solver-specific library environment variables.
Some examples are \texttt{MKL\_NUM\_THREADS}, \texttt{ulimit},  \texttt{OMP\_NUM\_THREADS}, and \texttt{I\_MPI\_JOB\_RESPECT\_PROCESS\_PLACEMENT}.

Two allocation methods were supported through the submission configuration - (a) resources are allocated and entrant code is launched on all the process ranks at the same time using an srun command or (b)  resources are allocated using an salloc and then entrant code is launched only on the first process rank. In the second case, it would be up to the entrant code to distribute its work across the allocated resources. The second option was mostly required by Julia codes using the Distributed package.
At any given time, there were as many as 250 nodes in full utilization running a number of entrant scenarios simultaneously.

\subsection{Team Performance}
\label{S:EntrantPerf}
The teams worked through the details of the challenge itself as well as making their code work on the competition platform.  Container systems like Docker and Singularity were planned, but not implemented due to security issues, Linux kernel versioning, and the challenges associated with MPI-based parallel computing using a variety of programming languages. The teams had to work through their challenges stemming either from their algorithmic logic or platform issues and these are listed in Table \ref{T:TeamChallengesT}. On the other hand, the organizers encountered several challenges and those are listed in \ref{T:OrganizerChallenges}.

\begin{longtable}{|p{5cm}|p{5cm}|p{5cm}|}
\caption{Team Challenges}\label{T:TeamChallengesT} \\
 \hline
\endhead
\small
    Out of memory (OOM): Some teams faced memory allocation issues during their runs, especially while dealing with large network models. Some of these even caused a couple of compute nodes to crash. &
    Segmentation fault: Some executable submissions were prone to segmentation faults on the Competition platform, but not on teams' own systems. This could be attributed to race conditions that manifest differently on different machines. These conditions can be notoriously hard to reproduce. &
    Convergence issues: These issues were solely attributable to teams' quality of algorithms. If their logs were comprehensive enough, tracing these issues was reasonable. \\
\hline
    Premature rank 0 exits: An MPI application typically has a rank 0 that does all the coordination and consolidation with   other processes. Rank 0 ensures that other processes exit before finally exiting itself. Some teams had issues with this logic and ended up in a state of incomplete solution files leading to slack scores. &
    Dataset formatting issues: Once in a while, teams had issues with parsing the datasets. There was a contention that competition was about developing the best algorithms and not necessarily the best dataset  parsers. This triggered some revisits to the datasets. An example is the use of comments and scientific notation in the text input files. &
    Julia errors: Julia does dynamic precompilation based on timestamp changes. A precompile cache is generated and modified when it goes stale. There were challenges around making different versions of Julia work for a number of teams and simultaneous scenario runs. Added to this, there were architectural differences between Julia versions as the language was evolving rapidly during a short time. \\
\hline
    Forking from an MPI application: Some teams attempted at launching solver executables like IPOPT or CPLEX from their MPI codes. Forking from MPI applications, especially with Open MPI implementation is strongly discouraged. Some scenario runs ended up in crash or other corrupted memory states. &
    
    OS-Library mismatches: Some solver libraries such as PARDISO were not built for the architecture and OS version that the Competition was hosted on. This caused team codes to fail, especially when they tried to supply the libraries themselves through the submission process.  At times executables targeted for a different OS or an advanced version of the hosted OS were submitted leading to launch failures. & \\
\hline
\end{longtable}



For the Final Event, there were seven  Python, four C++  and five each of Julia, executable binaries and MATLAB submissions. Nearly 70,000 scenarios runs were executed across Trial and Final events spanning 16 million CPU-hours and more than 200 PB of data. Counting the individual codes and evaluation runs, the total number of queued tasks were on the order of 200,000. 

\subsection{Requirements, Challenges, and Solutions}
 \label{S:Lessons}

There were several expectations and requirements set forth by the sponsor in order to conduct a fair and litigation-free Competition. These requirements, challenges with meeting these requirements and implemented solutions to handle the challenges are described in this section.

\begin{longtable}{|p{3cm}|p{6cm}|p{6cm}|}
\caption{Requirements, Challenges, and Resolutions } \label{T:OrganizerChallenges}\\
\hline
\multicolumn{1}{|l|}{Requirement/Expectation}   & \multicolumn{1}{l}{Platform Challenges} & \multicolumn{1}{|l|}{Resolution}		\\
\hline
\endhead
Entrants must have access to run logs and timely communication regarding progress of their runs. &

 Run duration ranges from few minutes to a few hours. It can be valuable if entrants can troubleshoot their problems without having to wait for hours. &

 Tail command is used to capture last few lines of all log files, concatenated, and placed on a webserver for every five minutes. A URL is provided for entrants to monitor them. They are allowed to terminate a run if anomalies are found. \\

\midrule

At times, there is a need to run scenarios for an event and simultaneously allow entrants to make submissions. &

The workflow for both approaches is different. Entrants are allowed to submit only one scenario at a time. Event scenarios have hundreds of scenarios for an entrant to be run. The scenarios themselves are sometimes restricted only to the event. The number of available cluster nodes need to be balanced between both the types. &
 The submission identifier was suffixed with flags to identify run types, perform load balancing, and route through distinct workflow appropriately. Additional criteria were set in place to ensure only permitted scenarios were run. \\
\midrule

 Scenarios that run well on entrant machines should also run with similar expectations on Competition platform. &
This is not always the case. Race conditions can manifest unsymmetrically on different machines. Differences in clusters (memory size and speed, cache sizes, etc.) and SLURM versions can cause anomalies. &

Exporting environment variables such as ulimit,  OMP\_NUM \_THREADS, MKL etc. sometimes made a difference though this was not required on entrant machines. At times, troubleshooting these was cumbersome requiring back and forth communication. \\
\midrule

Runtime duration of rerun scenarios must be more or less the same barring some acceptable variability. &

The potential culprits were  network traffic jams and the disks. Computing cluster nodes were networked through Infiniband for low latency and large bandwidth.  The shared drive accessible from all compute nodes was itself an independent set of disks. Yet, there were resource contention issues when a large number of scenario runs were running simultaneously. &

These issues with large variability in execution runtimes were traced to a few disks with bad sectors in the aging cluster. These were  replaced with new solid state disks. \\
\midrule

No two team’s scenarios and any two scenarios of a team should interfere during execution. &

 Shared Julia Depot \cite{bezanson2017julia} often ran into stale cache and interfered with other runs. &

 Distinct Julia depots were created for each team. All packages were precompiled. The scenario runs were invoked with “--compile-modules=no” feature on the Julia command line. \\
\midrule

 Teams should be given choice of MPI implementation. &

 A single installation of Python allows only one implementation of MPI. There are multiple versions of Python, multiple flavors of MPI, and multiple versions of MPI implementations. &

 Individual Python Virtual Environments were created to fulfill each requirement. \\
\midrule

C++ sources need to be compiled first and on the fly following a submission. &

 Schedulers disburse multiple scenarios simultaneously for execution. It is not in the best interest to recompile the same sources for every scenario. &

 During the first scenario, sources are compiled. The submission is marked  as an executable and then a flag is raised for other scenarios to get scheduled.  \\
\midrule

 Entrants should be able to submit executables. &

 The Competition hosting platform runs on Redhat 6.6 and has trouble running executables targeted for advanced Operating Systems (OS). &

 Executables built against Redhat 7.x were automatically detected and run against a set of compatible libraries on Redhat 6.6. Teams using other OS were requested to use container systems (e.g. Singularity) to produce target executables. \\

\bottomrule
\end{longtable}



A number of  trial events were conducted prior to the final competition event. They provided important lessons about the necessity of time limits, flexible runtime configuration, competitors stepping on each other (a Julia problem with shared depots), etc. Timing for MATLAB was problematic and the MATLAB Parallel Server did not scale well on the computing cluster. It often took several submission tries working closely systems personnel to achieve the correct specifications, but once set was quite reliable. The Competition platform has 4 new Nvidia DGX A100s each with 8 A100 GPUs and 1 TB of memory. There were  some inquiries but no team got to the stage of trying to run on GPUs. A good use of the Exabyte storage system was done on the platform.


Hardware failures were tracked using system logs and the corresponding run were automatically requeued and rerun. Scenarios that timed out with no results were automatically rerun once. Runs that resulted in bad or infeasible results within the time limit were generally not rerun unless there was reason to suspect resource contention issues, $i.e.$, similar runs on other scenarios were successful. Clusters of failures in a given time frame raised resource issue flags as well. Occasionally we would pin the 6 nodes in use to a specific switch where the full hardware bandwidth was available between nodes, but this rarely changed the results, indicating the most common contention issue was a combination of network and/or disk access contention.

The full cluster had over 500 nodes and as many as 250 were reserved for the exclusive use of the GO Competition which queued 3 tasks (code 1, code2, and Evaluation) for each scenario separately. During the year Challenge 1 was running we queued over 200,000 tasks from 70,000 scenarios and used 16 million CPU-hours (wall clock) while generating over 200 Petabytes of data.


